Forgetting and consolidation for incremental and cumulative knowledge acquisition systems

The application of cognitive mechanisms to support knowledge acquisition is, from our point of view, crucial for making the resulting models coherent, efficient, credible, easy to use and understandable. In particular, there are two characteristic features of intelligence that are essential for knowledge development: forgetting and consolidation. Both plays an important role in knowledge bases and learning systems to avoid possible information overflow and redundancy, and in order to preserve and strengthen important or frequently used rules and remove (or forget) useless ones. We present an incremental, long-life view of knowledge acquisition which tries to improve task after task by determining what to keep, what to consolidate and what to forget, overcoming The Stability-Plasticity dilemma. In order to do that, we rate rules by introducing several metrics through the first adaptation, to our knowledge, of the Minimum Message Length (MML) principle to a coverage graph, a hierarchical assessment structure which treats evidence and rules in a unified way. The metrics are not only used to forget some of the worst rules, but also to set a consolidation process to promote those selected rules to the knowledge base, which is also mirrored by a demotion system. We evaluate the framework with a series of tasks in a chess rule learning domain.

==> 4-Previous.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}\label{sec:related}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%TRANSFER LEARNING & RL%%%%


\emph{Lifelong Maching Learning}, or LML, a relatively new area of machine learning research, faces the problem of learning multiple consecutive tasks which is of great importance to the creation of intelligent, general-purpose, and  flexible machines.  According to Thrun \cite{Thrun96survey}, LML is concerned with the persistent and cumulative nature of learning, namely, a LML system must be: $(a)$ capable of retaining and using prior knowledge, and $(b)$ capable of acquiring new knowledge over a series of prediction tasks,  in order to improve the effectiveness (more accurate hypotheses) and efficiency (shorter training times) of learning. This subsection reviews some prior work on LML, mainly focused in Machine Learning areas where there have been some progress in knowledge retention, inductive transfer and forgetting procedures. 


Early work on lifelong learning was focused in the ML area of \emph{Transfer Learning} \cite{Pan10surveyTL}. Thrun in a series of papers \cite{Thrun96cluster,Mitchell93EBNNrobots,Thrun96survey}, focused on measures of task relatedness and sharing distance metrics to develop the \emph{Task Clustering} algorithm (TC) \cite{Thrun96cluster} with the aim of accelerating the learning of sets of related (same input space) binary classification tasks. TC employs a nearest neighbor classifier and transfers knowledge across multiple learning tasks by learning a distance metric for some tasks, and re-using it for learning in others. In contrast, our approach is a more general and flexible algorithm that do not work with a task-to-task mapping and supports the transfer of learning by composing effective cost-based background knowledge beyond just information provided as part of the examples and which, depending on the inductive engine used, is vital to both forming the hypothesis space and guiding the search. Furthermore our approach is meant for multiclass problems. 



%%%% RL %%%%


Furthermore, lifelong learning has also been explored for reinforcement learning either by learning incrementally or exploiting past learning experiences focusing on statistics, but given always an a well-developed and restricted sequence of possible environments. Ring \cite{Ring97child} developed CHILD, an agent capable of \emph{Continual}, \emph{Hierarchical}, \emph{Incremental Learning} and \emph{Development} with has no ultimate, final task. He combined the well-known Q-learning \cite{watkins92a} with the \emph{Temporal Transition Hierarchies} (TTH) \cite{Ring93learningsequential} learning algorithm, %a constructive neural-network-based learning system introduced as a continual-learning method for non-Markov reinforcement domains 
that allow a learning agent to build a hierarchy of skills (new behaviors are composed from variations on old ones) incrementally based on the temporal context. Tanaka et al. \cite{Tanaka97} and extended in \cite{Tanaka03,Tanaka03b} also proposed a lifelong machine learning approach for autonomous-robots (what they call \emph{Lifelong Reinforcement Learning}) by treating multiple environments as multiple-tasks. In this case the tasks to solve have some relations in common, and, when the learner faces the $n-th$ task, it employs the knowledge gathered through the previous $n-1$ tasks (as bias) which have been solved as individual tasks. % The systems uses the \emph{stochastic gradient method}, a type of memory-less reinforcement learning for unknown non-Markovian environment. 
 In this method, the policy is modeled by an artificial neural network where, as the bias, the authors focused on the variable range of each weight throughout the $n$ tasks. %: the average weight is used as initial bias (in each node); the dispersion of weights is used as learning bias as tunning parameter for the learning rate ($\alpha$) of each weigh. 
Our work, though, is a rule-based approach arranged with a \emph{coverage graph} where knowledge, unlike the previous approaches, is not a black box where its internals cannot be understood or manipulated but the opposite. Furthermore, the learned knowledge is not only seen as an increase or update of the previously learned knowledge (i.e. new behaviors are composed from variations on old ones), but as a constant review (including forgetting) of this knowledge based on its usefulness in order to deal with the new knowledge acquired which can be redundant or inconsistent with the consolidated one.



%%%% MTL %%%

Recently, Multiple task learning (MTL) \cite{Baxter00amodel, Caruana93multitasklearning} has also been considered to lifelong learning through the use of neural networks where the network is simultaneously trained on related classification tasks to improve generalisation in order to maximise the performance through shared knowledge. In the other cases, feed-forward networks are trained on one classification task and then modified and reused on a different classification: Thrun et al.\cite{Thrun96neural} also worked on a lifelong learning approached they called \emph{explanation-based neural networks} (EBNN). Originally proposed in the context of reinforcement learning \cite{Mitchell93EBNNrobots}, EBNNs are a neural network analogue to symbolic \emph{explanation-based learning} methods (EBL) \cite{Dejong86EBL,Mitchel86EBL}. EBNN uses standard back-propagation neural networks and, in order to transfer knowledge, EBNNs estimate the \emph{slopes} (tangents) to extract additional knowledge of the training set and exploits domain knowledge of previous learning tasks (back-propagation gradients of prior learned tasks) to guide the generalisation of the new one.  Silver et al. proposed variants of sequential learning and consolidation systems using standard back-propagation neural networks \cite{silver02,silver04,Silver96theparallel,Silver06cs} and introduced the \emph{task rehearsal method} (TRM) which uses the representation of previously learned tasks (virtual training examples generated by previous learned hypothesis) as a source of inductive bias and overcomes the problem of retaining specific training examples of early learning. The authors claimed that neural networks are the best option to transfer learning between related tasks due to its ability to capture regularities in the examples and to overcome the \emph{stability-plasticity} dilemma by using two neural networks (for short-term learning and long-term consolidation). Our work can also be seen as an example of MTL in which several different functions are learned together. However, unlike the previous approaches, our current approach uses a simpler strategy of revision (forgetting) and consolidation of knowledge which is also able to address the \emph{stability-plasticity} dilemma in a longlife learning process just by constantly evaluate and arrange the rules based on their complexity and compression through the use of a graph of deductive dependencies between rules. We see how the system is able to keep the useful rules and perform differently when new tasks can take advantage of the knowledge that has been consolidated from previous tasks. Furthermore, to our knowledge, this is the first general and comprehensive framework for life-long machine learning that can be applied to a diversity of rule-based learning systems.
 



Closer to our approach we find ELLA (Efficient Lifelong Learning Algorithm) \cite{ruvolo13} and NELL (Never-Ending Language Learner) \cite{Carlson10} which are another approaches to LML. The first one being a parametric approach based on the use of a \emph{shared basis} for all task models to improve learning over a set of tasks This method assume that each model is represented as a parameter vector that is a linear combination of these bases. By using a common basis, these approaches share information between learning tasks and account for task relatedness as the models are learned in tandem with the basis. As each new task arrives, ELLA transfers knowledge through the shared basis to learn the new model, and refines the basis with knowledge from the new task. This method incorporates aspects of both transfer and multi-task learning. The latter approach is and attempt of building a massive structured knowledge base. The system uses a semi-supervised multiple task learning approach composed by four subsystems which can read from the KB and consult other external resources (e.g., text corpora or the Internet): NELL starts  by training classifiers using a small amount of labeled data, then uses these classifiers to label unlabeled data (``candidate facts''). The most confident new labels are added to the KB (candidate facts promoted to ``beliefs'') used to train the models, and the process repeats. This iterative training is constrained with restrictions about which  candidates and promotions are allowable. Nonetheless, despite all these approaches are able to consolidate knowledge within a long-term domain knowledge structure, they do not introduce forgetting mechanisms that could eliminate obsolete knowledge.



%%%Theory revision%%%%

There are also connections with the area of theory revision, but in our case we do not look for semantic inconsistencies that could eventually be fixed, but just apply complexity-based metrics to the rules and see which of them are better and which are discardable. In fact, the ability of discarding irrelevant knowledge has been recognised as an important feature for knowledge based systems with approaches related to variable elimination in propositional and first-order logic \cite{Lang:2010:RUI:1824823.1824881,DBLP:journals/jair/WangZZZ14,AAAI113481}. This paper defines a general framework for reasoning from inconsistent propositional bases by introducing forgetting mechanisms. In comparison with our approach, this system is not addressed to the dynamic framework of life-long learning.



%%%%Graphs %%%

From a very different point of view, and since our approximation follows a graph representation and the idea that information on the graph could be ordered in a hierarchy by "node optimality", our work is also highly influenced by those problems related to link analysis in web graphs such as the HITS algorithm \cite{Kleinberg:1999:HITS}, PageRank \cite{Brin:1998:ALH:297810.297827} or SALSA \cite{Lempel:2000:SAL:346241.346324}. These algorithms share a common basis: the ranking vector they look for is the dominant eigenvector of a non-negative matrix (which definition differs in each method) that describes the link structure of the given network. 






